Hierarchical and Multimodal Data for Daily Activity Understanding

Daily Activity Recordings for Artificial Intelligence (DARai, pronounced "Dahr-ree") is a multimodal, hierarchically annotated dataset constructed to understand human activities in real-world settings. DARai consists of continuous scripted and unscripted recordings of 50 participants in 10 different environments, totaling over 200 hours of data from 20 sensors including multiple camera views, depth and radar sensors, wearable inertial measurement units (IMUs), electromyography (EMG), insole pressure sensors, biomonitor sensors, and gaze tracker. To capture the complexity in human activities, DARai is annotated at three levels of hierarchy: (i) high-level activities (L1) that are independent tasks, (ii) lower-level actions (L2) that are patterns shared between activities, and (iii) fine-grained procedures (L3) that detail the exact execution steps for actions. The dataset annotations and recordings are designed so that 22.7% of L2 actions are shared between L1 activities and 14.2% of L3 procedures are shared between L2 actions. The overlap and unscripted nature of DARai allows counterfactual activities in the dataset. Experiments with various machine learning models showcase the value of DARai in uncovering important challenges in human-centered applications. Specifically, we conduct unimodal and multimodal sensor fusion experiments for recognition, temporal localization, and future action anticipation across all hierarchical annotation levels. To highlight the limitations of individual sensors, we also conduct domain-variant experiments that are enabled by DARai's multi-sensor and counterfactual activity design setup. The code, documentation, and dataset are available at the dedicated DARai website: https://alregib.ece.gatech.edu/software-and-datasets/darai-daily-activity-recordings-for-artificial-intelligence-and-machine-learning/

==> Tables/confusion_matrixes.tex <==
\begin{figure}[h]
\normalsize
    \centering
    \begin{subfigure}{.5\textwidth}
        \centering
        \includegraphics[width=.8\linewidth]{figures/cm_emg.png}
        \caption{EMG data with ResNet-34 GAF Images}
        \label{fig:emgl1}
    \end{subfigure}%
    \begin{subfigure}{.5\textwidth}
        \centering
        \includegraphics[width=.8\linewidth]{figures/cm_imu.png}
        \caption{IMU data with ResNet-34 GAF Images}
        \label{fig:imul1}
    \end{subfigure}
    \begin{subfigure}{.5\textwidth}
        \centering
        \includegraphics[width=.8\linewidth]{figures/cm_gaze.png}
        \caption{Gaze data with ResNet-34 GAF Images}
        \label{fig:gazel1}
    \end{subfigure}%
    \begin{subfigure}{.5\textwidth}
        \centering
        \includegraphics[width=.8\linewidth]{figures/cm_insole.png}
        \caption{Insole data with ResNet-34 GAF Images}
        \label{fig:insolel1}
    \end{subfigure}
    \begin{subfigure}{.5\textwidth}
        \centering
        \includegraphics[width=.8\linewidth]{figures/cm_bio.png}
        \caption{Biomonitor data with ResNet-34 GAF Images}
        \label{fig:biol1}
    \end{subfigure}%
    \begin{subfigure}{.5\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/confusion_matrix_single-random_seed 1_ep 10_B 16 T 16_limited set_cam_1.png}
        \caption{RGB data with R3D model}
        \label{fig:rgbl1}
    \end{subfigure}
    \begin{subfigure}{.5\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/confusion_matrix_depth_single-random_seed 42_ep 10_B 16 T 16_limited set_depth_1.png}
        \caption{Depth data with R3D model}
        \label{fig:depthl1}
    \end{subfigure}%
    \begin{subfigure}{.5\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/rgbd_confusion_matrix_single-random_seed 1_ep 2_B 16 T 16_limited set_cam_1.png}
        \caption{RGB + Depth data with R3D model}
        \label{fig:rgbd}
    \end{subfigure}
    \caption{Confusion Matrix for unimodal and multimodal experiments}
\end{figure}

==> Tables/l1_visual_results.tex <==
\begin{table}[!h]
\centering
\scriptsize
\begin{tabular}{@{}cccccc@{}}
\toprule
\multicolumn{6}{c}{ Average Class Accuracy of L1 Activities for visual data}   
\\ \midrule
\multicolumn{1}{c}{Data Modalities} & \multicolumn{1}{c}{Training Model} & \multicolumn{1}{c}{View} &\multicolumn{1}{c}{Living Room} & \multicolumn{1}{c}{Kitchen} & \multicolumn{1}{c}{All Environments} \\
\midrule

RGB    &   R3D & $cam_1$  &  0.95 &0.67& 0.84   \\
RGB    &   R3D &  $cam_2$ &  0.90 &0.71 &0.89   \\
RGB    &   mvit\_v2\_s & $cam_1$  & 0.88 & 0.86 & 0.91     \\
RGB    &   mvit\_v2\_s &  $cam_2$ &  0.96 & 0.64 & 0.80     \\
RGB    &   swin3d\_t &  $cam_1$ & 0.90& 0.83 & 0.94    \\
RGB    &   swin3d\_t &  $cam_2$&      0.89 & 0.56 & 0.94\\
Depth &    R3D & $cam_1$ &   0.79 & 0.82 & 0.80  \\
Depth &    R3D &  $cam_2$ & & &   \\


\bottomrule
\end{tabular}
\vspace*{.1mm}
\caption{Unimodal video understanding benchmark results on L1 labels (Activities)}
\label{tab:l1_visual_result}
\end{table}

==> Tables/modalitycombination_info.tex <==
\begin{table}[h]
\centering
\caption{Information Provided by Modality Combinations}
\begin{tabular}{|l|p{8cm}|}
\hline
\textbf{Modality Combination} & \textbf{Information Provided} \\ \hline
RGB + D & Visual appearance, depth perception, spatial information \\ \hline
IMU + Bio & Body motion dynamics combined with physiological states \\ \hline
IMU + EMG & Motion dynamics, muscle activity, fine motor movements \\ \hline
IMU + Gaze & Body movement combined with focus direction \\ \hline
IMU + Insole & Combined lower body movements and stability \\ \hline
EMG + Insole & Muscle exertion and weight distribution for movement analysis \\ \hline
EMG + Gaze & Muscle activity combined with visual attention tracking \\ \hline
EMG + Bio & Muscle exertion combined with physiological signals \\ \hline
Insole + Gaze & Weight distribution combined with focus direction for stability analysis \\ \hline
Insole + Bio & Weight distribution, posture, and physiological signals \\ \hline
Gaze + Bio & Visual attention combined with physiological states for intent estimation \\ \hline
IMU + EMG + Insole + Bio & Comprehensive body motion, muscle activity, posture, and physiological analysis \\ \hline
IMU + EMG + Insole + Bio + Gaze & Holistic activity understanding combining motion, muscle, posture, physiology, and attention tracking \\ \hline
\end{tabular}
\label{tab:modality-combinations}
\end{table}

==> Tables/multimodal_result.tex <==

\begin{table}[!h]
\centering
\footnotesize
\begin{tabular}{@{}ccccc@{}}
\toprule
\multicolumn{5}{c}{ Average Class Accuracy}   
\\ \midrule
\multicolumn{1}{c}{Data Modalities} & \multicolumn{1}{c}{Training Model} & \multicolumn{1}{c}{Living Room} & \multicolumn{1}{c}{Kitchen} & \multicolumn{1}{c}{All Environments} \\
\midrule


\bottomrule
\end{tabular}
\vspace*{.1mm}
\caption{ Multimodal benchmark results of L1 labels (Activities) for different modalities}
\label{tab:uni_rgb-d}
\end{table}

==> Tables/observations.tex <==
{\scriptsize
\begin{longtable}{l p{5in}}
\toprule
\textbf{Topic} & \textbf{Key Findings} \\
\midrule
\multirow{3}{1in}{Sensors Setup }
& Sensor sampling rates vary significantly (from 15 fps to 1000 Hz), leading to substantial differences in data density. High-frequency sensors (e.g., EMG , Biomonitors) offer dense temporal resolution, beneficial for capturing fine-grain interactions and changes, whereas lower-frequency sensors (e.g., cameras at 15 fps) yield sparse data suited for broader spatial and temporal relations within activities. \\
 % \cmidrule(lr){1-2}
\midrule
 \multirow{3}{1in}{Hierarchical Annotations}
 % & In naturally occurring human activities, transitions between actions often lack clearly defined boundaries. Unlike structured datasets with predefined segmentation, DARai captures continuous activity sequences, where the start and end of specific actions or procedures emerge dynamically. \texttt{DARai} provides an opportunity of studying how models can handle real-world activity transitions and temporal uncertainty. \\
 & Natural human activities often lack certain boundaries between actions. Unlike structured datasets with predefined segments, \texttt{DARai} captures continuous activities with fluid transitions. It allows studying model performance on realistic temporal uncertainty and activity transitions. \\
 \cmidrule(lr){1-2}
 % \midrule
 \multirow{3}{1in}{Subjects }
 &  Participants experienced more fatigue than dehydration after performing daily activity in our data collection. \\
 & Participants rated the eye tracker as most obtrusive among sensors used, while insoles were rated the least noticeable, suggesting insoles may be the optimal sensor choice for minimizing wearer discomfort. \\
 % \cmidrule(lr){1-2}
 %  \multirow{3}{1in}{??? }
 % & ??? \\
 \cmidrule(lr){1-2}
 % \midrule
\multirow{3}{1in}{Visual Model Training Strategies}
 & Finetuned \emph{visual} models \emph{consistently outperform} those trained from scratch, across all class categories and all three levels of hierarchy. \\
 & Within kitchen and living room subsets, \emph{depth} models trained from scratch \emph{outperform} their RGB counterparts. \\
 & At levels L2 and L3 of the hierarchy, \emph{depth} models continue to outperform \emph{RGB} models trained from scratch, likely due to the stability of depth-based spatial representations across hierarchy levels. \\
\cmidrule(lr){1-2}
% \midrule
\multirow{1}{1in}{Environment Differences}
 & Activity recognition accuracy within the living room is \emph{consistently higher} than those within the kitchen. \\
\midrule

\multirow{3}{1in}{Viewpoint and Placement Effect}
 & Visual modalities suffer a \emph{severe drop} in accuracy when tested on the cross view. \\
 & Non-visual modalities are \emph{robust} when the sensors capture symmetric interaction such as insole. \\
 & Wearable cross-body models show \emph{less performance degradation} when compared to cross-view camera models. \\
\midrule

\multirow{6}{1in}{Unimodal Sensor Strengths}
 & Insole data effectively captures unique foot pressure patterns and performs well in recognizing activities such as \textsf{Carrying objects}. \\
 & IMU data are effective at separating activities with \emph{dynamic movements} such as \textsf{Exercising} from static activities such as \textsf{Working on a computer}. However, IMU data are less effective in separating activities with similar hand movements such as \textsf{Cleaning dishes} and \textsf{Cleaning the kitchen}. \\
 & Gaze data are effective at separating activities with \emph{explicit visual fixations} such as \textsf{Reading}, \textsf{Watching TV}, or \textsf{Working on a computer}. \\
 & Gaze data are effective at \emph{separating fine-grained activities} when other data modalities that rely on physical movements suffer from performance degradation. \\
 & EMG signals are proficient at identifying \emph{distinctive patterns of muscle interactions} and can consequently recognize activities such as \textsf{Making pancakes} (beating with a whisking motion) or \textsf{Playing video games} (repetitive controller grasping). Yet they have difficulty with activities such as \textsf{Making coffee}, where limited arm or hand interactions are used. \\
 & Bio-monitoring data are good at \emph{identifying changes in physiology}, such as increased heart rate in \textsf{Playing video games} or reduced activity in \textsf{Sleeping}. However, they lack the resolution to separate activities with similar effort, such as different cooking activities. \\
\midrule

\multirow{5}{1in}{Hierarchical Granularity}
 & Changes in performance across granularity levels are \emph{not} linear. \\
 & The visual model with the highest accuracy, \(\sim 56\%, \sim 59\%\), experiences a \emph{significant performance drop} when transitioning from L1 to L2 and L3. \\
 & Insole pressure and Hand EMG data modalities do \emph{not} exhibit a significant decline in performance from L1 to L2 as visual data does. \\
 & All modality combinations experience a decline in accuracy from L1 to L3, but the magnitude of degradation \emph{varies significantly} by sensor modality combination. \\
 & Gaze data improves L3 (procedure) activity recognition fused with other modalities. \\
 & Biomonitoring signals do not offer fine-grained insights at Level 3, even when combined with insole, EMG, and IMU data modalities. \\
\midrule

\multirow{2}{1in}{Temporal Localization}
 & In temporal activity localization, both the camera view and the length of the input video play a crucial role in accurately segmenting an untrimmed, abstract-level activity sample into lower-level segments. \\
 & Actions and procedures are not isolated events. They are interconnected components of larger sequences, with a strong dependence on the temporal context of those that come before and after. \\
\midrule

\multirow{5}{1in}{Short- and \ Long-Horizon Anticipation}
 & At L2 (Action level), a moderate observation period provides sufficient temporal context for immediate action anticipation, while excessive observation may introduce redundant or less relevant information. \\
 & Long-horizon anticipation at the L2 level, however, remains consistently lower and exhibits minimal improvement as the observation rate increases. This indicates that action-level predictions do not benefit significantly from extended temporal context, possibly due to the more independent nature of individual actions. \\
 & At the L3 (Procedure level), short-horizon anticipation improves as the observation rate increases, reaching optimal performance around a 70\% observation rate. \\
 & Long-horizon anticipation at this level consistently improves with increasing observation rates, eventually surpassing short-horizon performance beyond a 70\% observation rate. This trend suggests that fine-grained procedural activities exhibit stronger temporal dependencies, benefiting from longer observation windows that provide richer contextual information. \\
 & While higher observation rates do not necessarily enhance short-horizon anticipation, they are crucial for long-horizon anticipation, particularly when dealing with fine-grained, procedural activities. \\
\bottomrule
\caption{Key observations}
\label{tab:key_observations}
\end{longtable}
}

% \begin{table}[htb]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{l l l}
% \toprule
% \textbf{Section} & \textbf{Topic} & \textbf{Key Finding} \\
% \midrule
% (5.1) & \multirow{3}{*}{\centering Visual Training Strategies}
%       & Pretrained visual models consistently outperform those trained from scratch... \\
% (5.1) & & Within kitchen/living room, depth-from-scratch often outperforms RGB... \\
% (5.1) & & Depth remains competitive at L2 and L3 levels, suggesting more stable spatial representations... \\
% \midrule
% (5.1) & Environment Differences & Living room consistently achieves higher accuracy than kitchen... \\
% \midrule
% (5.2) & \multirow{3}{*}{\parbox{1in}{\centering Cross-View \\ and Cross-Body}} 
%       & Visual models suffer severe accuracy drop under cross-view... \\
% (5.2) & & Non-visual models are robust when sensors capture symmetric interactions (e.g., insole)... \\
% (5.2) & & Wearable cross-body models degrade less than cross-view camera models... \\
% \midrule
% (6.1) & \multirow{5}{*}{\parbox{1in}{\centering Unimodal Sensor Strengths}} 
%       & Insole data effectively captures foot pressure patterns (e.g., carrying objects)... \\
% (6.1) & & IMU data effectively separates highly dynamic vs.\ static activities, but struggles with similar hand movements... \\
% (6.1) & & Gaze data excels at activities with explicit visual fixations (reading, watching TV)... \\
% (6.1) & & EMG signals detect distinct muscle patterns (whisking vs.\ controller grasping), but fail on minimal movements... \\
% (6.1) & & Bio-monitoring captures physiological changes (heart rate) but lacks finer activity differentiation... \\
% \midrule
% (6.2) & \multirow{5}{*}{\centering Hierarchical Granularity}
%       & Performance changes from L1 to L2 to L3 are not linear... \\
% (6.2) & & Even the best visual model sees significant drop from L1 to deeper levels... \\
% (6.2) & & Non-visual modalities show a milder drop across levels... \\
% (6.2) & & All sensor combinations degrade from L1 to L3, but some more than others... \\
% (6.2) & & Certain modalities strongly boost fine-grained (L3) recognition... \\
% \midrule
% (7.1) & \multirow{2}{*}{\centering Temporal Activity Localization}
%       & Camera view and video length are critical for segmenting untrimmed activities... \\
% (7.1) & & Actions/procedures rely on interconnected temporal context, not isolation... \\
% \midrule
% (7.2) & \multirow{5}{*}{\centering Short vs. \\ Long-Horizon \\ Anticipation}
%       & At L2, short-horizon anticipation peaks at $\sim$50\% observed window, while long-horizon stays low... \\
% (7.2) & & Long-horizon at L2 offers minimal improvement with more observation... \\
% (7.2) & & At L3, short-horizon improves up to 70\% observed window... \\
% (7.2) & & Long-horizon at L3 steadily improves, surpassing short-horizon beyond 70\% observation... \\
% (7.2) & & While more observation does not always help short-horizon, it is key for long-horizon (especially fine-grained) tasks... \\
% \bottomrule
% \end{tabular}%
% }
% \caption{Key observations from each experimental setup, organized by shared topic.}
% \label{tab:key_observations_topics}
% \end{table}
\begin{comment}

\begin{table}[htb]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{l c p{8cm}}
% \begin{tabular}{lll}

\toprule
\textbf{Section} & \textbf{Topic} & \textbf{Key Finding} \\
\midrule

\multirow{4}{*}{(5.1)} & \multirow{3}{1in}{Visual Model Training Strategies}
 & pretrained visual models consistently outperform those trained from scratch. This trend holds across all class categories and across all three levels of the hierarchy. \\
 & & within the kitchen and living room subsets, depth models trained from scratch outperform their RGB counterparts. \\
 & & lower levels of the \texttt{DARai} hierarchy (L2 and L3), depth models continue to outperform RGB models trained from scratch, likely due to the stability of depth-based spatial representations across hierarchy levels. \\
\cmidrule(lr){2-3}
 & Environment Differences
 & activity recognition accuracy within the living room is consistently higher than those within the kitchen. \\
\midrule

\multirow{3}{*}{(5.2)} & \multirow{3}{1in}{Viewpoint and Placement Effect}
 & Visual models suffer a severe drop in accuracy when tested on the cross view. \\
 & & Non-visual models are more robust when the sensors capture symmetric interaction such as insole. \\
 & & wearable cross-body models show less performance degradation when compared to cross-view camera models. \\
\midrule

\multirow{6}{*}{(6.1)} & \multirow{6}{1in}{Unimodal Sensor Strengths}
 & insole data effectively captures unique foot pressure patterns and perform swell in recognizing activities such as \textsf{Carrying objects}. \\
 & & IMU data, which are effective at separating activities with dynamic movements such as \textsf{Exercising} and \textsf{Working on a computer}, which is a primarily static activity. However, IMU data are less effective in separating activities with similar hand movements such as \textsf{Cleaning dishes} and \textsf{Cleaning the kitchen}. \\
 & & Gaze data are effective at separating activities with explicit visual fixations such as "Reading," "Watching TV," or "Working on a computer." \\
 & & Gaze data are effective at separating fine grained activities when other data modalities that relies on physical movements suffer from performance degradation. \\
 & & EMG signals are proficient at identifying distinctive patterns of muscle interactions and can consequently recognize activities such as "Making pancakes" (beating with a whisking motion) or "playing video games" (repetitive controller grasping). Yet they have difficulty with activities such as "Making coffee" where limited arm or hand interactions are used. \\
 & & bio-monitoring data are good at identifying changes in physiology, such as increased heart rate in "playing video games" or reduced activity in "sleeping." However, they lack the resolution to separate activities with similar effort, such as different cooking activities. \\
\midrule

\multirow{5}{*}{(6.2)}  & \multirow{5}{1in}{Hierarchical Granularity}
 & changes in performance across granularity levels are \emph{not} linear. \\
 & & visual model with the highest accuracy, \(\sim 56\%, \sim 59\%\), experiences a significant performance drop when transitioning from L1 to L2 and L3. \\
 & & Non-visual modalities do not exhibit ta significant decline in performance from L1 to L2 and L3 as visual data does. \\
 & & all modality combinations experience a decline in accuracy from L1 to L3, but the magnitude of degradation varies significantly by sensor modality combination. \\
 & & highlights the strong contribution by a certain modality to fine-grain (L3) recognition. \\
\midrule

\multirow{2}{*}{(7.1)} & \multirow{2}{1in}{Temporal Activity Localization}
 & in temporal activity localization, both the camera view and the length of the input video play a crucial role in accurately segmenting an untrimmed, abstract-level activity sample into lower-level segments. \\
 & & actions and procedures are not learned in isolation but as interconnected components with a strong dependence on temporal context. \\
\midrule

\multirow{5}{*}{(7.2)} & \multirow{5}{1in}{Short vs.\ Long-Horizon Anticipation}
 & At L2 (Action level), short-horizon anticipation remains relatively stable, peaking at an observation rate of approximately 50\%, after which performance slightly declines. This suggests that a moderate observation period provides sufficient temporal context for immediate action anticipation, while excessive observation may introduce redundant or less relevant information. \\
 & & Long-horizon anticipation at the L2 level, however, remains consistently lower and exhibits minimal improvement as the observation rate increases. This indicates that action-level predictions do not benefit significantly from extended temporal context, possibly due to the more independent nature of individual actions. \\
 & & at the L3 (Procedure level), short-horizon anticipation improves as the observation rate increases, reaching optimal performance around 70\% observation rate. \\
 & & long-horizon anticipation at this level consistently improves with increasing observation rates, eventually surpassing short-horizon performance beyond 70\% observation rate. This trend suggests that fine-grained procedural activities exhibit stronger temporal dependencies, benefiting from longer observation windows that provide richer contextual information. \\
 & & while higher observation rates do not necessarily enhance short-horizon anticipation, they are crucial for long-horizon anticipation, particularly when dealing with fine-grained, procedural activities. \\
\bottomrule
\end{tabular} %
}
\caption{Key observations from each experimental setup, grouped by their main topic }
\label{tab:key_observations_topics}
\end{table}
\end{comment}   
\begin{comment}
   
\begin{table}[htb]
\centering
\footnotesize
\begin{tabularx}{\textwidth}{l c X}
\toprule
\textbf{Section} & \textbf{Topic} & \textbf{Key Finding} \\
\midrule

\multirow{4}{*}{(5.1)} & \multirow{3}{1in}{Visual Model Training Strategies}
 & pretrained visual models consistently outperform those trained from scratch. This trend holds across all class categories and across all three levels of the hierarchy. \\
 & & within the kitchen and living room subsets, depth models trained from scratch outperform their RGB counterparts. \\
 & & lower levels of the \texttt{DARai} hierarchy (L2 and L3), depth models continue to outperform RGB models trained from scratch, likely due to the stability of depth-based spatial representations across hierarchy levels. \\
\cmidrule(lr){2-3}
 & Environment Differences
 & activity recognition accuracy within the living room is consistently higher than those within the kitchen. \\
\midrule

\multirow{3}{*}{(5.2)} & \multirow{3}{*}{Viewpoint and Placement Effect}
 & Visual models suffer a severe drop in accuracy when tested on the cross view. \\
 & & Non-visual models are more robust when the sensors capture symmetric interaction such as insole. \\
 & & wearable cross-body models show less performance degradation when compared to cross-view camera models. \\
\midrule

\multirow{6}{*}{(6.1)} & \multirow{6}{*}{Unimodal Sensor Strengths}
 & insole data effectively captures unique foot pressure patterns and perform swell in recognizing activities such as \textsf{carrying objects}. \\
 & & IMU data, which are effective at separating activities with dynamic movements such as \textsf{Exercising} and \textsf{Working on a computer}, which is a primarily static activity. However, IMU data are less effective in separating activities with similar hand movements such as \textsf{Cleaning dishes} and \textsf{Cleaning the kitchen}. \\
 & & Gaze data are effective at separating activities with explicit visual fixations such as "Reading," "Watching TV," or "Working on a computer." \\
 & & Gaze data are effective at separating fine grained activities when other data modalities that relies on physical movements suffer from performance degradation. \\
 & & EMG signals are proficient at identifying distinctive patterns of muscle interactions and can consequently recognize activities such as "Making pancakes" (beating with a whisking motion) or "playing video games" (repetitive controller grasping). Yet they have difficulty with activities such as "Making coffee" where limited arm or hand interactions are used. \\
 & & bio-monitoring data are good at identifying changes in physiology, such as increased heart rate in "playing video games" or reduced activity in "sleeping." However, they lack the resolution to separate activities with similar effort, such as different cooking activities. \\
\midrule

\multirow{5}{*}{(6.2)}  & \multirow{5}{*}{Hierarchical Granularity}
 & changes in performance across granularity levels are \emph{not} linear. \\
 & & visual model with the highest accuracy, \(\sim 56\%, \sim 59\%\), experiences a significant performance drop when transitioning from L1 to L2 and L3. \\
 & & Non-visual modalities do not exhibit ta significant decline in performance from L1 to L2 and L3 as visual data does. \\
 & & all modality combinations experience a decline in accuracy from L1 to L3, but the magnitude of degradation varies significantly by sensor modality combination. \\
 & & highlights the strong contribution by a certain modality to fine-grain (L3) recognition. \\
\midrule

\multirow{2}{*}{(7.1)} & \multirow{2}{*}{Temporal Activity Localization}
 & in temporal activity localization, both the camera view and the length of the input video play a crucial role in accurately segmenting an untrimmed, abstract-level activity sample into lower-level segments. \\
 & & actions and procedures are not learned in isolation but as interconnected components with a strong dependence on temporal context. \\
\midrule

\multirow{5}{*}{(7.2)} & \multirow{5}{*}{Short vs.\ Long-Horizon Anticipation}
 & At L2 (Action level), short-horizon anticipation remains relatively stable, peaking at an observation rate of approximately 50\%, after which performance slightly declines. This suggests that a moderate observation period provides sufficient temporal context for immediate action anticipation, while excessive observation may introduce redundant or less relevant information. \\
 & & Long-horizon anticipation at the L2 level, however, remains consistently lower and exhibits minimal improvement as the observation rate increases. This indicates that action-level predictions do not benefit significantly from extended temporal context, possibly due to the more independent nature of individual actions. \\
 & & at the L3 (Procedure level), short-horizon anticipation improves as the observation rate increases, reaching optimal performance around 70\% observation rate. \\
 & & long-horizon anticipation at this level consistently improves with increasing observation rates, eventually surpassing short-horizon performance beyond 70\% observation rate. This trend suggests that fine-grained procedural activities exhibit stronger temporal dependencies, benefiting from longer observation windows that provide richer contextual information. \\
 & & while higher observation rates do not necessarily enhance short-horizon anticipation, they are crucial for long-horizon anticipation, particularly when dealing with fine-grained, procedural activities. \\
\bottomrule
\end{tabularx}
\caption{Key observations from each experimental setup, grouped by their main topic}
\label{tab:key_observations_topics}
\end{table}
\end{comment}

==> Tables/tab_modality_combination.tex <==

% % Optional: Force separation of floats
% \FloatBarrier



% \begin{table}[htbp]
% \centering
% \footnotesize
% \begin{tabular}{@{}p{4cm}p{4cm}p{1.5cm}} % cc@{}}
% \toprule
% \multicolumn{3}{c}{Performance Metrics for Multimodal Data Combinations} \\ \midrule
% \multicolumn{1}{c}{\textbf{Modality Combination}} & \multicolumn{1}{c}{\textbf{Information Provided}} & \multicolumn{1}{c}{\textbf{Performance}} \\ \midrule 

%     RGB + D & Visual appearance, depth perception, spatial information & & \\
%     \hline
%     IMU + Bio & Body motion dynamics combined with physiological states & & \\
%     \hline
%     IMU + EMG & Motion dynamics, muscle activity, fine motor movements & & \\
%     \hline
%     IMU + Gaze & Body movement combined with focus direction & & \\
%     \hline
%     IMU + Insole & Combined lower body movements and stability & & \\
%     \hline
%     EMG + Insole & Muscle exertion and Insole pressure distribution for movement analysis & & \\
%     \hline
%     EMG + Gaze & Muscle activity combined with visual gaze tracking & & \\
%     \hline
%     EMG + Bio & Muscle exertion combined with physiological signals & & \\
%     \hline
%     Insole + Gaze & Insole pressure distribution combined with focus direction for stability analysis & & \\
%     \hline
%     Insole + Bio & Insole pressure distribution, standing posture, and physiological signals & & \\
%     \hline
%     Gaze + Bio & Visual attention combined with physiological states for intent estimation & & \\
%     \hline
%     IMU + EMG + Insole + Bio & inertial motion and position, muscle activity, standing posture, and physiological signals & & \\
%     \hline
%     IMU + EMG + Insole + Bio + Gaze & Holistic activity understanding combining motion, muscle, standing posture, physiological signals, and gaze tracking & & \\
%     \hline
%     \bottomrule
% \end{tabular}
% \vspace*{.1mm}
% \caption{Summary of multimodal data combinations and their performance on L2 and L3 granularity levels.}
% \label{tab:modality_combinations}
% \end{table}

% Optional: Force separation of floats

\begin{table}[htbp]
\centering
\footnotesize
\begin{longtable}{@{}p{5cm}p{8cm}ccc@{}} % cc@{}}
\toprule
\multicolumn{5}{c}{Performance Metrics for Multimodal Data Combinations} \\ \midrule
\multicolumn{1}{c}{\textbf{Modality Combination}} & \multicolumn{1}{c}{\textbf{Information Provided}} & %\multicolumn{1}{c}{\textbf{Performance}} 
\multicolumn{3}{c}{\textbf{Performance}} \\
&& \textbf{L1} & \textbf{L2} & \textbf{L3}
\\ \midrule 

RGB + D & Visual appearance, depth perception, spatial information & & \\
\hline
IMU + Bio & Body motion dynamics combined with physiological states & 0.470 & 0.280 & 0.125 \\
\hline
IMU + EMG & Motion dynamics, muscle activity, fine-grain movements & 0.505 & 0.300 & 0.161 \\
\hline
IMU + Gaze & Motion dynamics combined with focus direction & 0.473 & 0.400 & 0.400 \\
\hline
IMU + Insole & Combined lower body movements and motion dynamics & 0.530 & 0.359 & 0.159 \\
\hline
EMG + Insole & Combined lower body movements and muscle activity & 0.405 & 0.400 & 0.073 \\
\hline
EMG + Gaze & Muscle activity combined with focus direction & 0.442 & 0.300 & 0.404 \\
\hline
EMG + Bio & Muscle activity combined with physiological signals & 0.368 & 0.200 & 0.026 \\
\hline
Insole + Gaze & Insole pressure distribution, lower body movements combined with focus direction & 0.461 & 0.340 & 0.410 \\
\hline
Insole + Bio & Insole pressure distribution, standing posture, and physiological signals & 0.391 & 0.300 & 0.070 \\
\hline
Gaze + Bio & Visual attention combined with physiological states & 0.416 & 0.240 & 0.390 \\
\hline
EMG + Insole + Bio & Muscle activity, insole pressure distribution, and physiological signals & 0.489 & 0.208 & 0.139 \\
\hline
IMU + Insole + Bio & Motion dynamics, insole stability, and physiological signals & 0.545 & 0.251 & 0.225 \\
\hline
IMU + EMG + Insole & Motion dynamics, muscle activity, and lower body movements & 0.535 & 0.281 & 0.220 \\
\hline
EMG + Insole + Gaze & Muscle activity, insole pressure distribution, and focus direction & 0.546 & 0.410 & 0.271 \\
\hline
IMU + Insole + Gaze & Motion dynamics, insole pressure distribution, and focus direction & 0.571 & 0.401 & 0.412 \\
\hline
IMU + EMG + Insole + Bio & Inertial motion and position, muscle activity, standing posture, and physiological signals & 0.556 & 0.322 & 0.233 \\
\hline
IMU + EMG + Insole + Bio + Gaze & Holistic activity understanding combining motion, muscle, standing posture, physiological signals, and focus tracking & 0.585 & 0.451 & 0.423 \\
\hline
\bottomrule
\end{longtable}
\vspace*{.1mm}
\caption{Summary of multimodal data combinations and their performance on L2 and L3 granularity levels.}
\label{tab:modality_combinations}
\end{table}


==> Tables/temporal-results/anticipation_result_20.tex <==
\begin{table}[!h]
\centering
\footnotesize
\begin{tabular}{@{}cccc@{}}
\toprule
\multicolumn{3}{c}{ Average MoF metric of L2 and L3 Classes for visual data}   
\\ \midrule
 \multicolumn{1}{c}{Model}  & \multicolumn{1}{c}{observed sequence length}  &\multicolumn{1}{c}{Anticipation Level: Action}\\
\midrule
   FUTR &  10\% & 52.854 \\
   FUTR &  20\% & 50.368 \\
   FUTR &  30\% & 42.910\\
   FUTR &  40\% &  35.294 \\
   FUTR &  50\% &  20.588 \\
   FUTR &  60\% &  20.588 \\
   FUTR &  70\% & 22.426 \\
   FUTR &  80\% & 16.176 \\
   FUTR &  90\% & 14.706 \\
%    TCN &   20\% &  28.309\\
%    TCN &   30\% &  34.191\\
%    TCN &   40\% &  33.456\\
%    TCN &   50\% &  35.662\\
%    TCN &   60\% &  32.721\\
%    TCN &   70\% &  30.882\\
%    TCN &   80\% &  20.343\\
%    TCN &   90\% &  20.931\\

\bottomrule
\multicolumn{1}{c}{}  & \multicolumn{1}{c}{}  &\multicolumn{1}{c}{Anticipation Level: Procedure}\\
\midrule
   FUTR &  20\% & 22.304 \\
   FUTR &  30\% & 24.958 \\
   FUTR &  40\% &  16.544 \\
   FUTR &  50\% &  23.389 \\
   FUTR &  60\% &  15.858 \\
   FUTR &  70\% & 16.544 \\
   FUTR &  80\% & 7.966 \\
   FUTR &  90\% & 7.353 \\
\bottomrule
\end{tabular}
\vspace*{.1mm}
\caption{Granular Action and Procedure Anticipation of Each Activity Sample}
\label{tab:anticipation_result}
\end{table}


==> Tables/temporal-results/anticipation_result_30.tex <==
\begin{table}[!h]
\centering
\footnotesize
\begin{tabular}{@{}cccc@{}}
\toprule
\multicolumn{3}{c}{ Average MoF metric of L2 and L3 Classes for visual data}   
\\ \midrule
 \multicolumn{1}{c}{Model}  & \multicolumn{1}{c}{observed sequence length}  &\multicolumn{1}{c}{Anticipation Level: Action}\\
\midrule
   FUTR &  10\% & 36.309 \\
   FUTR &  20\% & 42.121 \\
   FUTR &  30\% & 42.804\\
   FUTR &  40\% &  34.558 \\
   FUTR &  50\% &  35.661 \\
   FUTR &  60\% &  34.191 \\
   FUTR &  70\% & 27.941 \\
   FUTR &  80\% & 22.058 \\
   FUTR &  90\% & 15.294 \\
%    TCN &   20\% &  28.309\\
%    TCN &   30\% &  34.191\\
%    TCN &   40\% &  33.456\\
%    TCN &   50\% &  35.662\\
%    TCN &   60\% &  32.721\\
%    TCN &   70\% &  30.882\\
%    TCN &   80\% &  20.343\\
%    TCN &   90\% &  20.931\\

\bottomrule
\multicolumn{1}{c}{}  & \multicolumn{1}{c}{}  &\multicolumn{1}{c}{Anticipation Level: Procedure}\\
\midrule
   FUTR &  20\% & 22.304 \\
   FUTR &  30\% & 24.958 \\
   FUTR &  40\% &  16.544 \\
   FUTR &  50\% &  23.389 \\
   FUTR &  60\% &  15.858 \\
   FUTR &  70\% & 16.544 \\
   FUTR &  80\% & 7.966 \\
   FUTR &  90\% & 7.353 \\
\bottomrule
\end{tabular}
\vspace*{.1mm}
\caption{Granular Action and Procedure Anticipation of Each Activity Sample}
\label{tab:anticipation_result}
\end{table}


==> Tables/temporal-results/anticipation_result_40.tex <==
\begin{table}[!h]
\centering
\footnotesize
\begin{tabular}{@{}cccc@{}}
\toprule
\multicolumn{3}{c}{ Average MoF metric of L2 and L3 Classes for visual data}   
\\ \midrule
 \multicolumn{1}{c}{Model}  & \multicolumn{1}{c}{observed sequence length}  &\multicolumn{1}{c}{Anticipation Level: Action}\\
\midrule
   FUTR &  10\% & 24.789 \\
   FUTR &  20\% & 30.094 \\
   FUTR &  30\% & 44.957\\
   FUTR &  40\% &  56.25 \\
   FUTR &  50\% &  55.147 \\
   FUTR &  60\% &  47.058 \\
   FUTR &  70\% & 46.323 \\
   FUTR &  80\% & 29.779 \\
   FUTR &  90\% & 25.956 \\
%    TCN &   20\% &  28.309\\
%    TCN &   30\% &  34.191\\
%    TCN &   40\% &  33.456\\
%    TCN &   50\% &  35.662\\
%    TCN &   60\% &  32.721\\
%    TCN &   70\% &  30.882\\
%    TCN &   80\% &  20.343\\
%    TCN &   90\% &  20.931\\

\bottomrule
\multicolumn{1}{c}{}  & \multicolumn{1}{c}{}  &\multicolumn{1}{c}{Anticipation Level: Procedure}\\
\midrule
   FUTR &  20\% & 22.304 \\
   FUTR &  30\% & 24.958 \\
   FUTR &  40\% &  16.544 \\
   FUTR &  50\% &  23.389 \\
   FUTR &  60\% &  15.858 \\
   FUTR &  70\% & 16.544 \\
   FUTR &  80\% & 7.966 \\
   FUTR &  90\% & 7.353 \\
\bottomrule
\end{tabular}
\vspace*{.1mm}
\caption{Granular Action and Procedure Anticipation of Each Activity Sample}
\label{tab:anticipation_result}
\end{table}


==> Tables/temporal-results/anticipation_result_50.tex <==
\begin{table}[!h]
\centering
\footnotesize
\begin{tabular}{@{}cccc@{}}
\toprule
\multicolumn{3}{c}{ Average MoF metric of L2 and L3 Classes for visual data}   
\\ \midrule
 \multicolumn{1}{c}{Model}  & \multicolumn{1}{c}{observed sequence length}  &\multicolumn{1}{c}{Anticipation Level: Action}\\
\midrule
   FUTR &  10\% & 13.725 \\
   FUTR &  20\% & 18.697 \\
   FUTR &  30\% & 38.235\\
   FUTR &  40\% &  48.897 \\
   FUTR &  50\% &  45.588 \\
   FUTR &  60\% &  47.058 \\
   FUTR &  70\% & 40.073 \\
   FUTR &  80\% & 27.941 \\
   FUTR &  90\% & 19.705 \\
%    TCN &   20\% &  28.309\\
%    TCN &   30\% &  34.191\\
%    TCN &   40\% &  33.456\\
%    TCN &   50\% &  35.662\\
%    TCN &   60\% &  32.721\\
%    TCN &   70\% &  30.882\\
%    TCN &   80\% &  20.343\\
%    TCN &   90\% &  20.931\\

\bottomrule
\multicolumn{1}{c}{}  & \multicolumn{1}{c}{}  &\multicolumn{1}{c}{Anticipation Level: Procedure}\\
\midrule
   FUTR &  20\% & 22.304 \\
   FUTR &  30\% & 24.958 \\
   FUTR &  40\% &  16.544 \\
   FUTR &  50\% &  23.389 \\
   FUTR &  60\% &  15.858 \\
   FUTR &  70\% & 16.544 \\
   FUTR &  80\% & 7.966 \\
   FUTR &  90\% & 7.353 \\
\bottomrule
\end{tabular}
\vspace*{.1mm}
\caption{Granular Action and Procedure Anticipation of Each Activity Sample}
\label{tab:anticipation_result}
\end{table}


==> Tables/temporal-results/anticipation_result_60.tex <==
\begin{table}[!h]
\centering
\footnotesize
\begin{tabular}{@{}cccc@{}}
\toprule
\multicolumn{3}{c}{ Average MoF metric of L2 and L3 Classes for visual data}   
\\ \midrule
 \multicolumn{1}{c}{Model}  & \multicolumn{1}{c}{observed sequence length}  &\multicolumn{1}{c}{Anticipation Level: Action}\\
\midrule
   FUTR &  10\% & 32.633 \\
   FUTR &  20\% & 39.285 \\
   FUTR &  30\% & 48.056\\
   FUTR &  40\% &  54.779 \\
   FUTR &  50\% &  50.367 \\
   FUTR &  60\% &  41.176 \\
   FUTR &  70\% & 35.294 \\
   FUTR &  80\% & 30.882 \\
   FUTR &  90\% & 33.361 \\
%    TCN &   20\% &  28.309\\
%    TCN &   30\% &  34.191\\
%    TCN &   40\% &  33.456\\
%    TCN &   50\% &  35.662\\
%    TCN &   60\% &  32.721\\
%    TCN &   70\% &  30.882\\
%    TCN &   80\% &  20.343\\
%    TCN &   90\% &  20.931\\

\bottomrule
\multicolumn{1}{c}{}  & \multicolumn{1}{c}{}  &\multicolumn{1}{c}{Anticipation Level: Procedure}\\
\midrule
   FUTR &  20\% & 22.304 \\
   FUTR &  30\% & 24.958 \\
   FUTR &  40\% &  16.544 \\
   FUTR &  50\% &  23.389 \\
   FUTR &  60\% &  15.858 \\
   FUTR &  70\% & 16.544 \\
   FUTR &  80\% & 7.966 \\
   FUTR &  90\% & 7.353 \\
\bottomrule
\end{tabular}
\vspace*{.1mm}
\caption{Granular Action and Procedure Anticipation of Each Activity Sample}
\label{tab:anticipation_result}
\end{table}


==> Tables/temporal-results/anticipation_result_70.tex <==
\begin{table}[!h]
\centering
\footnotesize
\begin{tabular}{@{}cccc@{}}
\toprule
\multicolumn{3}{c}{ Average MoF metric of L2 and L3 Classes for visual data}   
\\ \midrule
 \multicolumn{1}{c}{Model}  & \multicolumn{1}{c}{observed sequence length}  &\multicolumn{1}{c}{Anticipation Level: Action}\\
\midrule
   FUTR &  10\% & 29.079 \\
   FUTR &  20\% & 33.403 \\
   FUTR &  30\% & 38.865\\
   FUTR &  40\% &  43.75 \\
   FUTR &  50\% &  54.779 \\
   FUTR &  60\% &  47.794 \\
   FUTR &  70\% & 53.834 \\
   FUTR &  80\% & 44.128 \\
   FUTR &  90\% & 31.838 \\
%    TCN &   20\% &  28.309\\
%    TCN &   30\% &  34.191\\
%    TCN &   40\% &  33.456\\
%    TCN &   50\% &  35.662\\
%    TCN &   60\% &  32.721\\
%    TCN &   70\% &  30.882\\
%    TCN &   80\% &  20.343\\
%    TCN &   90\% &  20.931\\

\bottomrule
\multicolumn{1}{c}{}  & \multicolumn{1}{c}{}  &\multicolumn{1}{c}{Anticipation Level: Procedure}\\
\midrule
   FUTR &  20\% & 22.304 \\
   FUTR &  30\% & 24.958 \\
   FUTR &  40\% &  16.544 \\
   FUTR &  50\% &  23.389 \\
   FUTR &  60\% &  15.858 \\
   FUTR &  70\% & 16.544 \\
   FUTR &  80\% & 7.966 \\
   FUTR &  90\% & 7.353 \\
\bottomrule
\end{tabular}
\vspace*{.1mm}
\caption{Granular Action and Procedure Anticipation of Each Activity Sample}
\label{tab:anticipation_result}
\end{table}


==> Tables/temporal-results/anticipation_result_80.tex <==
\begin{table}[!h]
\centering
\footnotesize
\begin{tabular}{@{}cccc@{}}
\toprule
\multicolumn{3}{c}{ Average MoF metric of L2 and L3 Classes for visual data}   
\\ \midrule
 \multicolumn{1}{c}{Model}  & \multicolumn{1}{c}{observed sequence length}  &\multicolumn{1}{c}{Anticipation Level: Action}\\
\midrule
   FUTR &  10\% & 36.309 \\
   FUTR &  20\% & 47.373 \\
   FUTR &  30\% & 41.071\\
   FUTR &  40\% &  40.073 \\
   FUTR &  50\% &  38.235 \\
   FUTR &  60\% &  47.058 \\
   FUTR &  70\% & 43.277 \\
   FUTR &  80\% & 39.999 \\
   FUTR &  90\% & 39.215 \\
%    TCN &   20\% &  28.309\\
%    TCN &   30\% &  34.191\\
%    TCN &   40\% &  33.456\\
%    TCN &   50\% &  35.662\\
%    TCN &   60\% &  32.721\\
%    TCN &   70\% &  30.882\\
%    TCN &   80\% &  20.343\\
%    TCN &   90\% &  20.931\\

\bottomrule
\multicolumn{1}{c}{}  & \multicolumn{1}{c}{}  &\multicolumn{1}{c}{Anticipation Level: Procedure}\\
\midrule
   FUTR &  20\% & 22.304 \\
   FUTR &  30\% & 24.958 \\
   FUTR &  40\% &  16.544 \\
   FUTR &  50\% &  23.389 \\
   FUTR &  60\% &  15.858 \\
   FUTR &  70\% & 16.544 \\
   FUTR &  80\% & 7.966 \\
   FUTR &  90\% & 7.353 \\
\bottomrule
\end{tabular}
\vspace*{.1mm}
\caption{Granular Action and Procedure Anticipation of Each Activity Sample}
\label{tab:anticipation_result}
\end{table}


==> Tables/temporal-results/anticipation_result_90.tex <==
\begin{table}[!h]
\centering
\footnotesize
\begin{tabular}{@{}cccc@{}}
\toprule
\multicolumn{3}{c}{ Average MoF metric of L2 and L3 Classes for visual data}   
\\ \midrule
 \multicolumn{1}{c}{Model}  & \multicolumn{1}{c}{observed sequence length}  &\multicolumn{1}{c}{Anticipation Level: Action}\\
\midrule
   FUTR &  10\% & 19.292 \\
   FUTR &  20\% & 26.313 \\
   FUTR &  30\% & 27.205\\
   FUTR &  40\% &  41.911 \\
   FUTR &  50\% &  39.338 \\
   FUTR &  60\% &  43.014 \\
   FUTR &  70\% & 48.529 \\
   FUTR &  80\% & 47.373 \\
   FUTR &  90\% & 54.642 \\
%    TCN &   20\% &  28.309\\
%    TCN &   30\% &  34.191\\
%    TCN &   40\% &  33.456\\
%    TCN &   50\% &  35.662\\
%    TCN &   60\% &  32.721\\
%    TCN &   70\% &  30.882\\
%    TCN &   80\% &  20.343\\
%    TCN &   90\% &  20.931\\

\bottomrule
\multicolumn{1}{c}{}  & \multicolumn{1}{c}{}  &\multicolumn{1}{c}{Anticipation Level: Procedure}\\
\midrule
   FUTR &  20\% & 22.304 \\
   FUTR &  30\% & 24.958 \\
   FUTR &  40\% &  16.544 \\
   FUTR &  50\% &  23.389 \\
   FUTR &  60\% &  15.858 \\
   FUTR &  70\% & 16.544 \\
   FUTR &  80\% & 7.966 \\
   FUTR &  90\% & 7.353 \\
\bottomrule
\end{tabular}
\vspace*{.1mm}
\caption{Granular Action and Procedure Anticipation of Each Activity Sample}
\label{tab:anticipation_result}
\end{table}


==> Tables/temporal-results/anticipation_result_v1.tex <==
\begin{table}[!h]
\centering
\footnotesize
\begin{tabular}{@{}cccc@{}}
\toprule
\multicolumn{3}{c}{ Average MoF metric of L2 and L3 Classes for visual data}   
\\ \midrule
 \multicolumn{1}{c}{Model}  & \multicolumn{1}{c}{observed sequence length}  &\multicolumn{1}{c}{Anticipation Level: Action}\\
\midrule

   FUTR &  20\% & 54.727 \\
   FUTR &  30\% & 55.777\\
   FUTR &  40\% &  55.882 \\
   FUTR &  50\% &  52.206 \\
   FUTR &  60\% &  48.162 \\
   FUTR &  70\% & 47.426 \\
   FUTR &  80\% & 41.176 \\
   FUTR &  90\% & 41.029 \\
%    TCN &   20\% &  28.309\\
%    TCN &   30\% &  34.191\\
%    TCN &   40\% &  33.456\\
%    TCN &   50\% &  35.662\\
%    TCN &   60\% &  32.721\\
%    TCN &   70\% &  30.882\\
%    TCN &   80\% &  20.343\\
%    TCN &   90\% &  20.931\\

\bottomrule
\multicolumn{1}{c}{}  & \multicolumn{1}{c}{}  &\multicolumn{1}{c}{Anticipation Level: Procedure}\\
\midrule
   FUTR &  20\% & 22.304 \\
   FUTR &  30\% & 24.958 \\
   FUTR &  40\% &  16.544 \\
   FUTR &  50\% &  23.389 \\
   FUTR &  60\% &  15.858 \\
   FUTR &  70\% & 16.544 \\
   FUTR &  80\% & 7.966 \\
   FUTR &  90\% & 7.353 \\
\bottomrule
\end{tabular}
\vspace*{.1mm}
\caption{Granular Action and Procedure Anticipation of Each Activity Sample}
\label{tab:anticipation_result}
\end{table}



==> Tables/temporal-results/anticipation_result_v2.tex <==
\begin{table}[!h]
\centering
\footnotesize
\begin{tabular}{@{}cccc@{}}
\toprule
\multicolumn{3}{c}{ Average MoF metric of L2 and L3 Classes for visual data}   
\\ \midrule
 \multicolumn{1}{c}{Model}  & \multicolumn{1}{c}{observed sequence length}  &\multicolumn{1}{c}{Anticipation Level: Action}\\
\midrule

   FUTR &  20\% & 54.727 \\
   FUTR &  30\% & 55.777\\
   FUTR &  40\% &  55.882 \\
   FUTR &  50\% &  52.206 \\
   FUTR &  60\% &  48.162 \\
   FUTR &  70\% & 47.426 \\
   FUTR &  80\% & 41.176 \\
   FUTR &  90\% & 41.029 \\
%    TCN &   20\% &  28.309\\
%    TCN &   30\% &  34.191\\
%    TCN &   40\% &  33.456\\
%    TCN &   50\% &  35.662\\
%    TCN &   60\% &  32.721\\
%    TCN &   70\% &  30.882\\
%    TCN &   80\% &  20.343\\
%    TCN &   90\% &  20.931\\

\bottomrule
\multicolumn{1}{c}{}  & \multicolumn{1}{c}{}  &\multicolumn{1}{c}{Anticipation Level: Procedure}\\
\midrule
   FUTR &  20\% & 22.304 \\
   FUTR &  30\% & 24.958 \\
   FUTR &  40\% &  16.544 \\
   FUTR &  50\% &  23.389 \\
   FUTR &  60\% &  15.858 \\
   FUTR &  70\% & 16.544 \\
   FUTR &  80\% & 7.966 \\
   FUTR &  90\% & 7.353 \\
\bottomrule
\end{tabular}
\vspace*{.1mm}
\caption{Granular Action and Procedure Anticipation of Each Activity Sample}
\label{tab:anticipation_result}
\end{table}



==> Tables/temporal-results/segmentation_result_20.tex <==
\begin{table}[!h]
\centering
\footnotesize
\begin{tabular}{@{}cccc@{}}
\toprule
\multicolumn{3}{c}{ Average MoF metric of L2 and L3 Classes for visual data}   
\\ \midrule
 \multicolumn{1}{c}{Model}  & \multicolumn{1}{c}{observed sequence length}  &\multicolumn{1}{c}{Anticipation Level: Action}\\
\midrule
   FUTR &  10\% & 32.583 \\
   FUTR &  20\% & 43.499 \\
   FUTR &  30\% & 39.602\\
   FUTR &  40\% &  32.998 \\
   FUTR &  50\% &  19.048 \\
   FUTR &  60\% &  16.057 \\
   FUTR &  70\% & 10.047 \\
   FUTR &  80\% & 9.742 \\
   FUTR &  90\% & 9.503 \\
%    TCN &   20\% &  28.309\\
%    TCN &   30\% &  34.191\\
%    TCN &   40\% &  33.456\\
%    TCN &   50\% &  35.662\\
%    TCN &   60\% &  32.721\\
%    TCN &   70\% &  30.882\\
%    TCN &   80\% &  20.343\\
%    TCN &   90\% &  20.931\\

\bottomrule
\multicolumn{1}{c}{}  & \multicolumn{1}{c}{}  &\multicolumn{1}{c}{Anticipation Level: Procedure}\\
\midrule
   FUTR &  20\% & 22.304 \\
   FUTR &  30\% & 24.958 \\
   FUTR &  40\% &  16.544 \\
   FUTR &  50\% &  23.389 \\
   FUTR &  60\% &  15.858 \\
   FUTR &  70\% & 16.544 \\
   FUTR &  80\% & 7.966 \\
   FUTR &  90\% & 7.353 \\
\bottomrule
\end{tabular}
\vspace*{.1mm}
\caption{Granular Action and Procedure Anticipation of Each Activity Sample}
\label{tab:anticipation_result}
\end{table}


==> Tables/temporal-results/segmentation_result_30.tex <==
\begin{table}[!h]
\centering
\footnotesize
\begin{tabular}{@{}cccc@{}}
\toprule
\multicolumn{3}{c}{ Average MoF metric of L2 and L3 Classes for visual data}   
\\ \midrule
 \multicolumn{1}{c}{Model}  & \multicolumn{1}{c}{observed sequence length}  &\multicolumn{1}{c}{Anticipation Level: Action}\\
\midrule
   FUTR &  10\% & 29.866 \\
   FUTR &  20\% & 40.894 \\
   FUTR &  30\% & 42.078\\
   FUTR &  40\% &  41.672 \\
   FUTR &  50\% &  36.302 \\
   FUTR &  60\% &  31.386 \\
   FUTR &  70\% & 26.899 \\
   FUTR &  80\% & 26.727 \\
   FUTR &  90\% & 22.645 \\
%    TCN &   20\% &  28.309\\
%    TCN &   30\% &  34.191\\
%    TCN &   40\% &  33.456\\
%    TCN &   50\% &  35.662\\
%    TCN &   60\% &  32.721\\
%    TCN &   70\% &  30.882\\
%    TCN &   80\% &  20.343\\
%    TCN &   90\% &  20.931\\

\bottomrule
\multicolumn{1}{c}{}  & \multicolumn{1}{c}{}  &\multicolumn{1}{c}{Anticipation Level: Procedure}\\
\midrule
   FUTR &  20\% & 22.304 \\
   FUTR &  30\% & 24.958 \\
   FUTR &  40\% &  16.544 \\
   FUTR &  50\% &  23.389 \\
   FUTR &  60\% &  15.858 \\
   FUTR &  70\% & 16.544 \\
   FUTR &  80\% & 7.966 \\
   FUTR &  90\% & 7.353 \\
\bottomrule
\end{tabular}
\vspace*{.1mm}
\caption{Granular Action and Procedure Anticipation of Each Activity Sample}
\label{tab:anticipation_result}
\end{table}


==> Tables/temporal-results/segmentation_result_40.tex <==
\begin{table}[!h]
\centering
\footnotesize
\begin{tabular}{@{}cccc@{}}
\toprule
\multicolumn{3}{c}{ Average MoF metric of L2 and L3 Classes for visual data}   
\\ \midrule
 \multicolumn{1}{c}{Model}  & \multicolumn{1}{c}{observed sequence length}  &\multicolumn{1}{c}{Anticipation Level: Action}\\
\midrule
   FUTR &  10\% & 31.766 \\
   FUTR &  20\% & 31.499 \\
   FUTR &  30\% & 41.956\\
   FUTR &  40\% &  41.056 \\
   FUTR &  50\% &  43.551 \\
   FUTR &  60\% &  38.906 \\
   FUTR &  70\% & 35.116 \\
   FUTR &  80\% & 28.110 \\
   FUTR &  90\% & 24.169 \\
%    TCN &   20\% &  28.309\\
%    TCN &   30\% &  34.191\\
%    TCN &   40\% &  33.456\\
%    TCN &   50\% &  35.662\\
%    TCN &   60\% &  32.721\\
%    TCN &   70\% &  30.882\\
%    TCN &   80\% &  20.343\\
%    TCN &   90\% &  20.931\\

\bottomrule
\multicolumn{1}{c}{}  & \multicolumn{1}{c}{}  &\multicolumn{1}{c}{Anticipation Level: Procedure}\\
\midrule
   FUTR &  20\% & 22.304 \\
   FUTR &  30\% & 24.958 \\
   FUTR &  40\% &  16.544 \\
   FUTR &  50\% &  23.389 \\
   FUTR &  60\% &  15.858 \\
   FUTR &  70\% & 16.544 \\
   FUTR &  80\% & 7.966 \\
   FUTR &  90\% & 7.353 \\
\bottomrule
\end{tabular}
\vspace*{.1mm}
\caption{Granular Action and Procedure Anticipation of Each Activity Sample}
\label{tab:anticipation_result}
\end{table}


==> Tables/temporal-results/segmentation_result_50.tex <==
\begin{table}[!h]
\centering
\footnotesize
\begin{tabular}{@{}cccc@{}}
\toprule
\multicolumn{3}{c}{ Average MoF metric of L2 and L3 Classes for visual data}   
\\ \midrule
 \multicolumn{1}{c}{Model}  & \multicolumn{1}{c}{observed sequence length}  &\multicolumn{1}{c}{Anticipation Level: Action}\\
\midrule
   FUTR &  10\% & 20.686 \\
   FUTR &  20\% & 28.400 \\
   FUTR &  30\% & 36.455\\
   FUTR &  40\% &  41.896 \\
   FUTR &  50\% &  43.896 \\
   FUTR &  60\% &  47.958 \\
   FUTR &  70\% & 35.819 \\
   FUTR &  80\% & 40.081 \\
   FUTR &  90\% & 31.278 \\
%    TCN &   20\% &  28.309\\
%    TCN &   30\% &  34.191\\
%    TCN &   40\% &  33.456\\
%    TCN &   50\% &  35.662\\
%    TCN &   60\% &  32.721\\
%    TCN &   70\% &  30.882\\
%    TCN &   80\% &  20.343\\
%    TCN &   90\% &  20.931\\

\bottomrule
\multicolumn{1}{c}{}  & \multicolumn{1}{c}{}  &\multicolumn{1}{c}{Anticipation Level: Procedure}\\
\midrule
   FUTR &  20\% & 22.304 \\
   FUTR &  30\% & 24.958 \\
   FUTR &  40\% &  16.544 \\
   FUTR &  50\% &  23.389 \\
   FUTR &  60\% &  15.858 \\
   FUTR &  70\% & 16.544 \\
   FUTR &  80\% & 7.966 \\
   FUTR &  90\% & 7.353 \\
\bottomrule
\end{tabular}
\vspace*{.1mm}
\caption{Granular Action and Procedure Anticipation of Each Activity Sample}
\label{tab:anticipation_result}
\end{table}


==> Tables/temporal-results/segmentation_result_60.tex <==
\begin{table}[!h]
\centering
\footnotesize
\begin{tabular}{@{}cccc@{}}
\toprule
\multicolumn{3}{c}{ Average MoF metric of L2 and L3 Classes for visual data}   
\\ \midrule
 \multicolumn{1}{c}{Model}  & \multicolumn{1}{c}{observed sequence length}  &\multicolumn{1}{c}{Anticipation Level: Action}\\
\midrule
   FUTR &  10\% & 17.585 \\
   FUTR &  20\% & 25.716 \\
   FUTR &  30\% & 27.715\\
   FUTR &  40\% &  35.010 \\
   FUTR &  50\% &  42.536 \\
   FUTR &  60\% &  37.923 \\
   FUTR &  70\% & 29.361 \\
   FUTR &  80\% & 28.739 \\
   FUTR &  90\% & 31.125 \\
%    TCN &   20\% &  28.309\\
%    TCN &   30\% &  34.191\\
%    TCN &   40\% &  33.456\\
%    TCN &   50\% &  35.662\\
%    TCN &   60\% &  32.721\\
%    TCN &   70\% &  30.882\\
%    TCN &   80\% &  20.343\\
%    TCN &   90\% &  20.931\\

\bottomrule
\multicolumn{1}{c}{}  & \multicolumn{1}{c}{}  &\multicolumn{1}{c}{Anticipation Level: Procedure}\\
\midrule
   FUTR &  20\% & 22.304 \\
   FUTR &  30\% & 24.958 \\
   FUTR &  40\% &  16.544 \\
   FUTR &  50\% &  23.389 \\
   FUTR &  60\% &  15.858 \\
   FUTR &  70\% & 16.544 \\
   FUTR &  80\% & 7.966 \\
   FUTR &  90\% & 7.353 \\
\bottomrule
\end{tabular}
\vspace*{.1mm}
\caption{Granular Action and Procedure Anticipation of Each Activity Sample}
\label{tab:anticipation_result}
\end{table}


==> Tables/temporal-results/segmentation_result_70.tex <==
\begin{table}[!h]
\centering
\footnotesize
\begin{tabular}{@{}cccc@{}}
\toprule
\multicolumn{3}{c}{ Average MoF metric of L2 and L3 Classes for visual data}   
\\ \midrule
 \multicolumn{1}{c}{Model}  & \multicolumn{1}{c}{observed sequence length}  &\multicolumn{1}{c}{Anticipation Level: Action}\\
\midrule
   FUTR &  10\% & 27.510 \\
   FUTR &  20\% & 30.832 \\
   FUTR &  30\% & 38.530\\
   FUTR &  40\% &  48.283 \\
   FUTR &  50\% &  50.569 \\
   FUTR &  60\% &  46.314 \\
   FUTR &  70\% & 49.858 \\
   FUTR &  80\% & 41.795 \\
   FUTR &  90\% & 38.125 \\
%    TCN &   20\% &  28.309\\
%    TCN &   30\% &  34.191\\
%    TCN &   40\% &  33.456\\
%    TCN &   50\% &  35.662\\
%    TCN &   60\% &  32.721\\
%    TCN &   70\% &  30.882\\
%    TCN &   80\% &  20.343\\
%    TCN &   90\% &  20.931\\

\bottomrule
\multicolumn{1}{c}{}  & \multicolumn{1}{c}{}  &\multicolumn{1}{c}{Anticipation Level: Procedure}\\
\midrule
   FUTR &  20\% & 22.304 \\
   FUTR &  30\% & 24.958 \\
   FUTR &  40\% &  16.544 \\
   FUTR &  50\% &  23.389 \\
   FUTR &  60\% &  15.858 \\
   FUTR &  70\% & 16.544 \\
   FUTR &  80\% & 7.966 \\
   FUTR &  90\% & 7.353 \\
\bottomrule
\end{tabular}
\vspace*{.1mm}
\caption{Granular Action and Procedure Anticipation of Each Activity Sample}
\label{tab:anticipation_result}
\end{table}


==> Tables/temporal-results/segmentation_result_80.tex <==
\begin{table}[!h]
\centering
\footnotesize
\begin{tabular}{@{}cccc@{}}
\toprule
\multicolumn{3}{c}{ Average MoF metric of L2 and L3 Classes for visual data}   
\\ \midrule
 \multicolumn{1}{c}{Model}  & \multicolumn{1}{c}{observed sequence length}  &\multicolumn{1}{c}{Anticipation Level: Action}\\
\midrule
   FUTR &  10\% & 18.872 \\
   FUTR &  20\% & 38.438 \\
   FUTR &  30\% & 36.479\\
   FUTR &  40\% &  35.931 \\
   FUTR &  50\% &  36.859 \\
   FUTR &  60\% &  44.352 \\
   FUTR &  70\% & 37.261 \\
   FUTR &  80\% & 37.002 \\
   FUTR &  90\% & 34.064 \\
%    TCN &   20\% &  28.309\\
%    TCN &   30\% &  34.191\\
%    TCN &   40\% &  33.456\\
%    TCN &   50\% &  35.662\\
%    TCN &   60\% &  32.721\\
%    TCN &   70\% &  30.882\\
%    TCN &   80\% &  20.343\\
%    TCN &   90\% &  20.931\\

\bottomrule
\multicolumn{1}{c}{}  & \multicolumn{1}{c}{}  &\multicolumn{1}{c}{Anticipation Level: Procedure}\\
\midrule
   FUTR &  20\% & 22.304 \\
   FUTR &  30\% & 24.958 \\
   FUTR &  40\% &  16.544 \\
   FUTR &  50\% &  23.389 \\
   FUTR &  60\% &  15.858 \\
   FUTR &  70\% & 16.544 \\
   FUTR &  80\% & 7.966 \\
   FUTR &  90\% & 7.353 \\
\bottomrule
\end{tabular}
\vspace*{.1mm}
\caption{Granular Action and Procedure Anticipation of Each Activity Sample}
\label{tab:anticipation_result}
\end{table}


==> Tables/temporal-results/segmentation_result_90.tex <==
\begin{table}[!h]
\centering
\footnotesize
\begin{tabular}{@{}cccc@{}}
\toprule
\multicolumn{3}{c}{ Average MoF metric of L2 and L3 Classes for visual data}   
\\ \midrule
 \multicolumn{1}{c}{Model}  & \multicolumn{1}{c}{observed sequence length}  &\multicolumn{1}{c}{Anticipation Level: Action}\\
\midrule
   FUTR &  10\% & 22.253 \\
   FUTR &  20\% & 19.913 \\
   FUTR &  30\% & 30.440\\
   FUTR &  40\% &  34.514 \\
   FUTR &  50\% &  43.570 \\
   FUTR &  60\% &  53.287 \\
   FUTR &  70\% & 52.820 \\
   FUTR &  80\% & 54.228 \\
   FUTR &  90\% & 52.417 \\
%    TCN &   20\% &  28.309\\
%    TCN &   30\% &  34.191\\
%    TCN &   40\% &  33.456\\
%    TCN &   50\% &  35.662\\
%    TCN &   60\% &  32.721\\
%    TCN &   70\% &  30.882\\
%    TCN &   80\% &  20.343\\
%    TCN &   90\% &  20.931\\

\bottomrule
\multicolumn{1}{c}{}  & \multicolumn{1}{c}{}  &\multicolumn{1}{c}{Anticipation Level: Procedure}\\
\midrule
   FUTR &  20\% & 22.304 \\
   FUTR &  30\% & 24.958 \\
   FUTR &  40\% &  16.544 \\
   FUTR &  50\% &  23.389 \\
   FUTR &  60\% &  15.858 \\
   FUTR &  70\% & 16.544 \\
   FUTR &  80\% & 7.966 \\
   FUTR &  90\% & 7.353 \\
\bottomrule
\end{tabular}
\vspace*{.1mm}
\caption{Granular Action and Procedure Anticipation of Each Activity Sample}
\label{tab:anticipation_result}
\end{table}


==> Tables/unimodal.tex <==

\begin{table}[h]
\centering
\begin{tabular}{@{}cccc@{}}
\toprule
\multicolumn{4}{c}{ Average Class Accuracy for R3D Model}   
\\ \midrule
\multicolumn{1}{c}{Modalities} & \multicolumn{1}{c}{Living Room} & \multicolumn{1}{c}{Kitchen} & \multicolumn{1}{c}{All Environments} \\
\midrule

RGB    &       0.97       & 0.67            &   0.84     \\
Depth &      0.64     &   0.66      & 0.75    \\


\bottomrule
\end{tabular}
\vspace*{.1mm}
\caption{Benchmark results of video understanding of L1 labels (Activities) for unimodal RGB and Depth data across separate and combined classes in each environment}
\label{tab:uni_rgb-d}
\end{table}

==> Tables/unimodal_abalation.tex <==
\begin{tabular}{@{}p{3cm}p{4cm}p{2cm}@{}}
\toprule
\multicolumn{3}{c}{Uni-modal Performance Comparison Across Different Models} \\ \midrule
\multicolumn{1}{c}{\textbf{Data Modality}} & \multicolumn{1}{c}{\textbf{Model Architecture}} & \multicolumn{1}{c}{\textbf{Performance}} \\ \midrule

\multirow{3}{*}{RGB $view_1$} & R3d\_18 & 0.84 \\
                              & mvit small & 0.91 \\
                              & swin3d tiny & 0.94 \\ \midrule

\multirow{3}{*}{RGB $view_2$} & R3d\_18 & 0.89 \\
                              & mvit small & 0.8 \\
                              & swin3d tiny & 0.71 \\ \midrule

\multirow{3}{*}{Depth $view_1$} & R3d\_18 & 0.75 \\
                                & mvit small & 0.39 \\
                                & swin3d tiny & 0.65 \\\midrule

\multirow{3}{*}{Depth $view_2$} & R3d\_18 & 0.51 \\
                                & mvit small & 0.42 \\
                                & swin3d tiny & 0.37 \\ 
                                \midrule

\multirow{3}{*}{\textcolor{cyan}{IMU}} & Transformer & 0.42 \\
                     % & Resnet_34 & 0.43 \\
                     & LSTM & 0.32   \\
                     & BiLSTM & 0.32 \\ \midrule

\multirow{3}{*}{\textcolor{NavyBlue}{EMG}} & Transformer  & 0.30 \\
                     % & Resnet_34 & 0.46 \\
                     & LSTM & 0.14 \\
                     & BiLSTM & 0.14 \\ \midrule

\multirow{3}{*}{\textcolor{violet}{Insole}} & Transformer  & 0.37 \\
                        % & Resnet_34 & 0.42 \\
                        & LSTM & 0.18 \\
                     & BiLSTM & 0.12 \\ \midrule

\multirow{3}{*}{\textcolor{OliveGreen}{Bio}} & Transformer & 0.25 \\
                     % & Resnet_34 & 0.36 \\
                     & LSTM & 0.22 \\
                     & BiLSTM & 0.20 \\ \midrule

\multirow{3}{*}{\textcolor{orange}{Gaze}} & Transformer & 0.29 \\
                      % & Resnet_34 & 0.44 \\
                     & LSTM & 0.16 \\
                     & BiLSTM & 0.16 \\ 

\bottomrule
\end{tabular}
